Exact Detection Thresholds and Minimax Optimality of Chatterjee's Correlation Coefficient

Recently, Chatterjee (2021) introduced a new rank-based correlation coefficient which can be used to measure the strength of dependence between two random variables. This coefficient has already attracted much attention as it converges to the Dette-Siburg-Stoimenov measure (see Dette et al. (2013)), which equals $0$ if and only if the variables are independent and $1$ if and only if one variable is a function of the other. Further, Chatterjee's coefficient is computable in (near) linear time, which makes it appropriate for large-scale applications. In this paper, we expand the theoretical understanding of Chatterjee's coefficient in two directions: (a) First we consider the problem of testing for independence using Chatterjee's correlation. We obtain its asymptotic distribution under any changing sequence of alternatives converging to the null hypothesis (of independence). We further obtain a general result that gives exact detection thresholds and limiting power for Chatterjee's test of independence under natural nonparametric alternatives converging to the null. As applications of this general result, we prove a $n^{-1/4}$ detection boundary for this test and compute explicitly the limiting local power on the detection boundary for popularly studied alternatives in the literature. (b) We then construct a test for non-trivial levels of dependence using Chatterjee's coefficient. In contrast to testing for independence, we prove that, in this case, Chatterjee's coefficient indeed yields a minimax optimal procedure with a $n^{-1/2}$ detection boundary. Our proof techniques rely on Stein's method of exchangeable pairs, a non-asymptotic projection result, and information theoretic lower bounds.

==> hypernat <==
%% hypernat.sty v1.0b (C) 2001 Jens Berger
%%
%%  This packages makes the hyperref package and the natbib package
%%  with options `numbers' and `sort&compress' work together. This
%%  means, that the citations (e.g [3,2,1]) will be compressed to
%%  [1-3], where the `1' and the `3' are (color-)linked to the
%%  bibliography.
%%
%%  The changes I made here are suggested (in August 2000) for the
%%  next natbib release.
%%
%%  This package will disappear from CTAN, when natbib will do
%%  the job by himself.
%%
%%  Load this package after natbib and hyperref!
%%
%%  Please make sure that you are using at least natbib v7.0!
%%
%% Changes
%%
%%   v1.0b 2001/07/09 anchor for all citations in the list added 
%%                    to make backref options working (bug reported by Günter Keusen)
%%   v1.0a 2001/01/22 \noexpand for some \hyper@natlinkend added 
%%                    (bug reported by Frank Meißen), hypernat.sty 
%%                    is working now for `dvips --> ps2pdf' or `dvips -> Distiller'
%%
\ProvidesPackage{hypernat}[2001/07/09 v1.0b hyperref and natbib compatibility (jb)]
\AtBeginDocument{\def\NAT@sort{2}}
\def\NAT@citexnum[#1][#2]#3{%
  \NAT@sort@cites{#3}%
  \let\@citea\@empty
   \@cite{\def\NAT@num{-1}\let\NAT@last@yr\relax\let\NAT@nm\@empty
    \@for\@citeb:=\NAT@cite@list\do
    {\edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb\@extra@b@citeb}{%
       {\reset@font\bfseries?}
        \NAT@citeundefined\PackageWarning{natbib}%
       {Citation `\@citeb' on page \thepage \space undefined}}%
     {\let\NAT@last@num\NAT@num\let\NAT@last@nm\NAT@nm
      \NAT@parse{\@citeb}%
      \ifNAT@longnames\@ifundefined{bv@\@citeb\@extra@b@citeb}{%
        \let\NAT@name=\NAT@all@names
        \global\@namedef{bv@\@citeb\@extra@b@citeb}{}}{}%
      \fi
      \ifNAT@full\let\NAT@nm\NAT@all@names\else
        \let\NAT@nm\NAT@name\fi
      \ifNAT@swa
       \ifnum\NAT@ctype>1\relax\@citea
        \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
            \ifnum\NAT@ctype=2\relax\NAT@test{\NAT@ctype}%
            \else\NAT@alias
            \fi\hyper@natlinkend\else
       \ifnum\NAT@sort>1
         \begingroup\catcode`\_=8
            \ifcat _\ifnum\z@<0\NAT@num _\else A\fi
              \global\let\NAT@nm=\NAT@num \else \gdef\NAT@nm{-2}\fi
            \ifcat _\ifnum\z@<0\NAT@last@num _\else A\fi
              \global\@tempcnta=\NAT@last@num \global\advance\@tempcnta by\@ne
              \else \global\@tempcnta\m@ne\fi
         \endgroup
% v0.1b anchor added to make backref's working, watch for errors!
         \ifnum\NAT@nm=\@tempcnta
         \ifHy@backref\hyper@natlinkstart{\@citeb\@extra@b@citeb}\hyper@natlinkend\fi
           \ifx\NAT@last@yr\relax
%             \edef\NAT@last@yr{\@citea \mbox{\noexpand\citenumfont{\NAT@num}}}%
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
               \edef\NAT@last@yr{\@citea \mbox{\noexpand%
                    \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
                      \noexpand\citenumfont{\NAT@num}%
                    \noexpand\hyper@natlinkend}%
               }%
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           \else
%             \edef\NAT@last@yr{--\penalty\@m\mbox{\noexpand\citenumfont{\NAT@num}}}%
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
             \edef\NAT@last@yr{--\penalty\@m\mbox{\noexpand%
                  \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
                    \noexpand\citenumfont{\NAT@num}%
                  \noexpand\hyper@natlinkend}%
             }%
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           \fi
         \else
%           \NAT@last@yr \@citea \mbox{\citenumfont{\NAT@num}}%
           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           \NAT@last@yr \@citea \mbox{%
                \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
                    \citenumfont{\NAT@num}%
                \hyper@natlinkend}%
           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           \let\NAT@last@yr\relax
         \fi
       \else
         \@citea \mbox{\hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           {\citenumfont{\NAT@num}}\hyper@natlinkend}%
       \fi
       \fi
       \def\@citea{\NAT@sep\penalty\@m\NAT@space}%
      \else
        \ifcase\NAT@ctype\relax
          \ifx\NAT@last@nm\NAT@nm \NAT@yrsep\penalty\@m\NAT@space\else
          \@citea \NAT@test{1}\ \NAT@@open
          \if*#1*\else#1\ \fi\fi \NAT@mbox{%
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
          {\citenumfont{\NAT@num}}\hyper@natlinkend}%
          \def\@citea{\NAT@@close\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@test{\NAT@ctype}\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@test{\NAT@ctype}\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \or\@citea
          \hyper@natlinkstart{\@citeb\@extra@b@citeb}%
           \NAT@alias\hyper@natlinkend
          \def\@citea{\NAT@sep\penalty\@m\ }%
        \fi
      \fi
      }}%
      \ifnum\NAT@sort>1\relax\NAT@last@yr\fi
      \ifNAT@swa\else\ifnum\NAT@ctype=0\if*#2*\else
      \NAT@cmt#2\fi \NAT@@close\fi\fi}{#1}{#2}%
}
\endinput

